VAT-Mart: Learning Visual Action Trajectory Proposals for Manipulating 3D ARTiculated Objects

Perceiving and manipulating 3D articulated objects (e.g., cabinets, doors) in human environments is an important yet challenging task for future home-assistant robots. The space of 3D articulated objects is exceptionally rich in their myriad semantic categories, diverse shape geometry, and complicated part functionality. Previous works mostly abstract kinematic structure with estimated joint parameters and part poses as the visual representations for manipulating 3D articulated objects. In this paper, we propose object-centric actionable visual priors as a novel perception-interaction handshaking point that the perception system outputs more actionable guidance than kinematic structure estimation, by predicting dense geometry-aware, interaction-aware, and task-aware visual action affordance and trajectory proposals. We design an interaction-for-perception framework VAT-Mart to learn such actionable visual representations by simultaneously training a curiosity-driven reinforcement learning policy exploring diverse interaction trajectories and a perception module summarizing and generalizing the explored knowledge for pointwise predictions among diverse shapes. Experiments prove the effectiveness of the proposed approach using the large-scale PartNet-Mobility dataset in SAPIEN environment and show promising generalization capabilities to novel test shapes, unseen object categories, and real-world data. Project page: https://hyperplane-lab.github.io/vat-mart

==> tabs/stats_590.tex <==
\begin{table}[t]
\caption{We summarize the shape counts in our dataset. Here, \textit{Micro} and \textit{Washing} are short for microwave and washing machine.
  There are three data splits: training data from the training categories, test data from the training categories, and data from the test categories. We use the first split to train all networks and use the rest two for evaluation.}
  \vspace{2mm}
  \centering
  \setlength{\tabcolsep}{1pt}
  \renewcommand\arraystretch{0.5}
  \small
    \begin{tabular}{c|c|cccc|c|c}
    \toprule
    Train-Cats & \diagbox{\small{All}}{\small{Door}}   & \small{Cabinet} & \small{Door}   & \small{Mirco} & \small{Fridge} & \diagbox{\small{All}}{\small{Drawer}} & \small{Cabinet}  \\ 
    \midrule
    Train-Data & 337 & 270    & 23    & 11   & 33 & 270 & 270  \\
    \midrule
    Test-Data & 105   & 76    & 13    & 5 & 11 & 76 & 76 \\
    \toprule
    Test-Cats &    & \small{Safe}   & \small{Table} & \small{Washing} &   & & \small{Table}  \\
    \midrule
    Test-Data & 148 & 30 & 101 & 17 & & 101  & 101  \\
    \bottomrule
    \end{tabular}
  \label{tab:dataset_stats}
\end{table}%

==> tabs/succ2.tex <==
\begin{table*}[t]
  \centering
    \setlength{\tabcolsep}{5pt}
  \renewcommand\arraystretch{0.5}
  \small
% \begin{tabular}{@{}llcccccc@{}}
% \toprule
%   && Accuracy (\%) & Precision (\%) & Recall (\%) & F-score (\%) & Sample-Succ (\%) & Coverage (\%)  \\
% \midrule
% \multirow{5}{*}{pushing}
% & door &  6.83 / 3.99 & 50.00 / 50.00 & 12.02 / 7.40 & 50.00 / 50.00 & 50.00 / 50.00 & 6.80 / 3.79 \\
% & drawer & 19.75 / 9.89 & 83.48 / 71.63 & 31.94 / 17.39 & 75.12 / 72.87 & 79.30 / 72.25 & 21.72 / 11.57 \\
% & slider & 19.93 / 10.34 & 81.33 / 76.47 & 32.01 / 18.21 & 76.03 / 72.41 & 78.68 / 74.44 & 18.04 / 9.15 \\
% & switch & 26.29 / 15.14 & \textbf{88.46} / \textbf{84.08} & 40.54 / 25.66 & 81.82 / 80.40 & 85.14 / \textbf{82.24} & 25.18 / 11.76 \\
% \midrule
% \multirow{5}{*}{pulling}
% & door & 2.59 / 1.71 & 50.00 / 50.00 & 4.92 / 3.31 & 50.00 / 50.00 & 50.00 / 50.00 & 2.70 / 1.62 \\
% & drawer & 7.24 / 3.98 & 86.58 / 75.87 & 13.37 / 7.56 & 70.57 / 68.06 & 78.58 / 71.97 & 8.93 / 4.81 \\
% & slider & 8.33 / 3.98 & 79.92 / 65.42 & 15.08 / 7.50 & 76.65 / 72.45 & 78.29 / 68.93 & 8.09 / 4.86 \\
% & switch & 11.94 / \textbf{6.26} & 87.87 / \textbf{76.14} & 21.03 / \textbf{11.57} & 82.80 / 80.11 & 85.34 / \textbf{78.12} & \textbf{12.88} / 6.43 \\
% \bottomrule
% \end{tabular}
\begin{tabular}{@{}llcccccc@{}}
\toprule
& RL-baseline &  Heuristic & Ours without Curiosity & Ours with Curiosity &  &  &  \\
\midrule
pushing door
& w & 80.28 / 76.60 & 76.73 / 75.48 & 86.83 / 78.69 & 81.47 / 77.05 & 13.14 / 9.92 & 82.63 / 78.88 \\
\midrule
pulling door
& w & 75.82 / 76.89 & 69.76 / 74.62 & 88.52 / 81.51 & 78.02 / 77.91 & 4.80 / 3.36 & 55.26 / 50.76 \\
\midrule
pushing drawer
& w & 84.36 / 84.48 & 77.78 / 79.29 & 96.08 / 93.28 & 85.96 / 85.71 & 14.01 / 13.17 & 95.49 / 95.46 \\
\midrule
pulling drawer
& w & 87.96 / 90.48 & 88.60 / 90.25 & 87.11 /90.76 & 87.85 / 90.50 & 12.89 / 7.89 & 93.05 / 91.62 \\
\midrule
pushing slider
& w & 86.43 / 65.99 & 82.99 / 73.95 & 91.60 / 49.38 & 87.08 / 59.22 & 15.69 / * & 97.82 / 69.35 \\
\midrule
pulling slider
& w & 87.11 / 87.39 & 85.71 / 86.18 & 89.08 / 89.08 & 87.36 / 87.60 & 12.61 / * & 98.32 /88.29 \\
\bottomrule
\end{tabular}

  \caption{Quantitative evaluations on different tasks and metrics. \ruihai{no comparison with baselines}\kaichun{If no 5.3, we need to compare with no-curiosity for all, since no other baselines.}}
  \label{tab:results_full}
  \vspace{-4mm}
\end{table*}%%
